Data-free Universal Adversarial Perturbation with Pseudo-semantic Prior

Data-free Universal Adversarial Perturbation (UAP) is an image-agnostic adversarial attack that deceives deep neural networks using a single perturbation generated solely from random noise without relying on data priors. However, traditional data-free UAP methods often suffer from limited transferability due to the absence of semantic content in random noise. To address this issue, we propose a novel data-free universal attack method that recursively extracts pseudo-semantic priors directly from the UAPs during training to enrich the semantic content within the data-free UAP framework. Our approach effectively leverages latent semantic information within UAPs via region sampling, enabling successful input transformations-typically ineffective in traditional data-free UAP methods due to the lack of semantic cues-and significantly enhancing black-box transferability. Furthermore, we introduce a sample reweighting technique to mitigate potential imbalances from random sampling and transformations, emphasizing hard examples less affected by the UAPs. Comprehensive experiments on ImageNet show that our method achieves state-of-the-art performance in average fooling rate by a substantial margin, notably improves attack transferability across various CNN architectures compared to existing data-free UAP methods, and even surpasses data-dependent UAP methods. Code is available at: https://github.com/ChnanChan/PSP-UAP.

==> sec/0_abstract.tex <==
\begin{abstract}

Data-free Universal Adversarial Perturbation (UAP) is an image-agnostic adversarial attack that deceives deep neural networks using a single perturbation generated solely from random noise, without any data priors.
However, traditional data-free UAP methods often suffer from limited transferability due to the absence of semantic information in random noise.
To address this, we propose a novel data-free universal attack method that generates a pseudo-semantic prior recursively from the UAPs, enriching semantic contents within the data-free UAP framework.
Our method is based on the observation that UAPs inherently contain latent semantic information, enabling the generated UAP to act as an alternative data prior, by capturing a diverse range of semantics through region sampling.
We further introduce a sample reweighting technique to emphasize hard examples by focusing on samples that are less affected by the UAP.
% We further introduce a new sample reweighting method that emphasizes the losses of samples less affected by the UAP, thereby increasing the focus on hard examples.
By leveraging the semantic information from the pseudo-semantic prior, we also incorporate input transformations, typically ineffective in data-free UAPs due to the lack of semantic content in random priors, to boost black-box transferability.
Comprehensive experiments on ImageNet show that our method achieves state-of-the-art performance in average fooling rate by a substantial margin, significantly improves attack transferability across various CNN architectures compared to existing data-free UAP methods, and even surpasses data-dependent UAP methods.
Code is available at:~\url{https://github.com/ChnanChan/PSP-UAP}
% Furthermore, by leveraging the semantic information from the pseudo-Semantic Prior, we are able to incorporate input transformations—commonly used in image-specific adversarial methods but otherwise ineffective in data-free UAPs—to enhance black-box transferability.
% Furthermore, we adopt input transformation techniques widely used in image-specific adversarial perturbation methods, which are less explored in data-free UAP due to the lack of semantics in random priors, to boost transferability for black-box attacks.

% Furthermore, we adapt input transformation techniques  employed in data-dependent UAP methods, which are traditionally challenging to apply in data-free UAPs due to the lack of data, to boost transferability across black-box models. 
% To mitigate the adverse effects of overly strong transformations on UAP, we introduce an uncertainty-based re-weighting loss, that assigns greater weights to samples where the model predicts with high confidence.
%, allowing for intensive training on specific semantic priors.



\iffalse
Universal adversarial perturbation~(UAP) is an image-agnostic adversarial attack aiming to fool deep neural networks with a single perturbation across numerous data samples.
However, the adversary does not always know the target data domain, so data-free universal attacks generated from random noise have recently been attracted.
Conventional data-free universal attacks exhibit constrained transferability as they rely on random noise without any prior knowledge of the image dataset. %the target domain.
% Existing data-free universal attacks have low attack transferability since only maximize the CNN activation without any prior target domain.
%In this paper, we propose a method to enhance the semantic richness of random noise by leveraging the semantic properties of UAP to overcome the absence of prior knowledge.
In this paper, we introduce a novel data-free universal attack method called PSP-UAP that addresses the challenge of lacking a prior dataset by generating pseudo-semantic priors.
Specifically, we design an activation re-weighting loss to effectively leverage the diverse semantic information contained in the pseudo-semantic priors.
Furthermore, we adapt input transformation attack methods, which are typically difficult to apply directly to data-free UAPs, to enhance attack transferability across black-box models.
%Additionally, we utilize various augmentation techniques to provide the model with a more diverse set of semantic priors.
%The semantic priors generated through our method facilitate the progressive learning of UAP that specifically targets and disrupts patterns significantly activated by the model.
%In image-specific attacks, applying input transformation methods that allow the model to learn various variances can improve transferability, but it has not been tried in data-free settings due to a lack of input data.
%In this paper, we propose a novel data-free universal attack by generating auxiliary train data samples for UAP without target domain samples through random crop and resizing UAPs on the optimizing stage, which we call \textbf{R}andom c\textbf{R}op, \textbf{R}esize, \textbf{R}eplace, and \textbf{X}-transformation UAP (R4X-UAP).
%In this paper, we propose a novel data-free universal attack by generating auxiliary train data samples for UAP without target domain samples through random crop and resizing UAPs on the optimizing stage, which we call \textbf{R}andom c\textbf{R}op, \textbf{R}esize, \textbf{R}eplace, and \textbf{X}-transformation UAP (R4X-UAP).
%Furthermore, we adapt arbitrary input transformation attack methods to incorporate auxiliary data samples, thereby fully exploiting advantages that cannot be achieved by solely maximizing positive activation in convolution layers through the addition of random noise.
%Specifically, we design an activation re-weighting loss to effectively leverage the diverse semantic information contained in the pseudo-data samples.
Extensive experiments on the ImageNet dataset demonstrate that our PSP-UAP achieves a state-of-the-art average fooling rate and significantly enhances attack transferability on different CNN models as compared to other data-free universal attack methods.
\fi
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}


%-------------------------------------------------------------------------

Deep neural networks (DNNs) have become widely used in computer vision, achieving remarkable performance across a diverse range of tasks, such as image classification~\cite{res152, inc_v3}, object detection~\cite{yolo, faster}, semantic segmentation~\cite{u-net}, and visual tracking~\cite{siam, fairmot}.
Despite these successes, DNNs are vulnerable to carefully crafted, imperceptible perturbations in input data, causing the model to make highly confident yet incorrect predictions.
This vulnerability poses significant challenges for deploying DNNs in critical applications, such as autonomous driving~\cite{autonomous} and security systems~\cite{security}, and has led to increased research into adversarial attacks that generate adversarial examples.
% Despite these successes, research has shown that DNNs remain susceptible to imperceptible perturbations, which result in erroneous and unpredictable predictions.
% These potential risks heighten concerns regarding the deployment of DNNs and have led to an increased focus on researching adversarial attacks that generate adversarial examples (AEs).


%--------------------------c -----------------------------------------------

\begin{figure}[!t]
% \vspace{0.3cm}
\centering    \includegraphics[width=\linewidth]{figures/figure_1.pdf}
    \caption{ Diverse semantic contents in both a real-image and UAP: 
    {(a)} A whole image from the ImageNet dataset (top) and our generated data-free UAP (bottom) from DenseNet-121, shown at iteration 900 during the training phase. The Top-1 class and its score are shown below each image. 
    {(b)} Cropped regions from the whole image (top) and our UAP (bottom). Those regions contain diverse semantics that differ from the class of the original images.
    % \textbf{First columns:} ImageNet data and our PSP-UAP generated on DenseNet-121. \textbf{Other columns:} Images randomly cropped and resized to the original input size. Both cropped and resized images from UAP and real-world data show that even from the same original image, they have different top-1 labels.
    }
    % \vspace{-0.2cm}
    \label{fig:fig_1}
\end{figure}



To craft the adversarial examples with high transferability across various DNN architectures, there have been many adversarial attack methods using a specific target image~\cite{FGSM, Deepfool, mifgsm, l-bfgs, generating, i-fgsm}.
However, these methods generate a unique perturbation for each target image, which is time-consuming, impractical for real-world scenarios, and limits their generalization to other images.
To tackle this limitation, the Universal Adversarial Perturbation (UAP)~\cite{UAP} introduced an image-agnostic attack that generates a single image-agnostic adversarial perturbation, which is capable of attacking a wide range of unknown images.
Many studies~\cite{sga-uap, spgd, nag, gap} focus on developing data-dependent UAPs that target unknown models, thereby enhancing transferability across diverse and unseen scenarios.
While these UAPs deceive diverse categories of images with a single perturbation, they still rely on large-scale data samples and their labels from the target domain to capture diverse semantics, such as the ImageNet~\cite{Imagenet} dataset. 


% Since access to data priors from the target domain is not always feasible, data-free UAP methods~\cite{FFF, gd-uap, TRM, pd-ua, AAA} gain attention recently, which train UAPs using only random noise, without relying on any dataset.
Accessing data priors from the target domain is often impractical, leading to recent interest in data-free UAP methods~\cite{FFF,gd-uap,TRM,pd-ua,AAA,at-uap,cosine}.
% , which train UAPs from random noise without any dataset. 
Data-free UAP poses a greater challenge than conventional data-dependent UAP generation tasks, as it restricts the employment of any prior knowledge of the target domain dataset.
Prior works~\cite{FFF, gd-uap, TRM} have attempted to craft UAPs from random noise without any dataset, by maximizing activations in convolutional neural networks (CNNs) layers. 
% the feature level of convolutional neural networks (CNNs) by maximizing the activation of convolutional layers. 
However, these methods solely rely on random priors, such as Gaussian noise or jigsaw patterns, which lack semantic information and thus offer limited transferability to unseen models.
To overcome this limitation, several works~\cite{AAA, at-uap} utilize auxiliary data samples generated by optimizing against the outputs of a surrogate model.
Although these methods allow the use of semantic information in synthetic data, the crafted UAPs often show inferior transferability due to overfitted data to the surrogate model.
% To tackle this issue, some works~\cite{AAA, at-uap} leverage auxiliary data samples generated by optimizing with the outputs of the surrogate model.
% However, these often overfit the surrogate model, limiting the transferability of the crafted UAP.
% Optimizing auxiliary dataset~\cite{AAA, at-uap} often overfits the surrogate model, limiting the transferability of the crafted UAP.
% ~\cite{FFF, gd-uap, cosine, TRM, pd-ua}
%Additionally, current data-free UAP methods primarily utilize activations from the surrogate model’s convolutional layers, further restricting transferability to black-box models.


% In this paper, we explore how to leverage semantic information without any dataset priors, using only the UAP itself, to mitigate these issues.
In this paper, we explore how to leverage semantic information directly from the UAP itself, without any dataset priors, to address these challenges.
Our approach is inspired by the observation that even a single generated UAP contains diverse semantic information as well as its dominant label, as shown in Figure~\ref{fig:fig_1}.
We find that the generated UAP encodes diverse semantic features, similar to a real-world image with various semantic contents across different regions.
% We observe that the generated UAP holds diverse semantic features, similar to a real-world image that contains various semantics when examining different parts. 
For example, in Figure~\ref{fig:fig_1}, while the whole UAP is predicted as `Safe' due to its tendency to have a dominant label, cropped regions within the UAP are predicted as classes like `Brain coral,' `Puck,' and `Slot.' 
This observation motivates us to utilize UAP as a semantic prior for training within a data-free UAP framework.
% This observation leads us to the idea of using UAPs as a semantic prior during training within a data-free UAP framework.


% Inspired by this, we propose PSP-UAP, a novel data-free UAP method that leverages UAPs, treated as data prior with various semantic information, alongside random noise to generate pseudo-semantic priors during training, that mitigates the limitations of data-free constraints for training UAP.
% This allows for the use of more diverse activated regions and various semantic information to deceive the model more effectively despite lacking the prior dataset.
% Inspired by this, we propose PSP-UAP, a novel data-free UAP method that uses UAPs as data priors with diverse semantic information, combined with random noise, to generate pseudo-semantic priors during training.
Inspired by this insight, we propose a novel data-free UAP method, called PSP-UAP, which generates pseudo-semantic priors from a UAP during training.
% which combines a UAP with random noise to generate pseudo-semantic priors during training.
%that combines UAPs containing diverse semantic information with random noise to generate pseudo-semantic priors during training.
% This approach addresses the data-free constraint in UAP generation by incorporating richer semantic information, rather than random noise, within UAPs.
To capture more diverse semantics in pseudo-semantic priors, we randomly crop and resize regions to extract semantic samples and treat them as images to fool. 
This approach effectively addresses the data-free constraint in UAP generation by leveraging richer semantic information inherent in the UAP, rather than relying solely on random noise.
% This approach addresses the limitation of data-free constraint in UAP generation by incorporating more diverse activated regions and richer semantic information within UAPs, enabling more effective model deception, even without access to prior datasets.
% \chany{This approach addresses the data-free constraint in UAP generation by incorporating richer semantic information, rather than random noise, within UAPs.}
% enabling more effective model deception. %, even without access to prior datasets.}
% However, randomly cropped pseudo-semantic priors may have uninformative samples, and averaging the activations of these samples equally disrupts the generation of an optimal UAP.
However, randomly cropped semantic samples often vary in informativeness, and simply averaging their activations can disrupt the generation of an optimal UAP.
% However, randomly cropped semantic samples are often inconsistently informative, and equally averaging the activations of these samples disrupts the generation of an optimal UAP.
% To address this, we introduce a sample reweighting loss to focus more on hard examples less deceived by an attack with a current UAP.
To mitigate this problem, we introduce a sample reweighting to focus on hard examples less deceived by an attack with a current UAP.
% We also incorporate input transformations~\cite{xie2019improving,L2T} into our data-free UAP framework to improve transferability across models, a technique commonly applied in image-specific adversarial attacks. 
To further improve the attack transferability, we incorporate input transformations~\cite{xie2019improving, L2T}, primarily used in image-specific adversarial attacks, into our data-free UAP framework.
% This approach remains unexplored in data-free UAPs, as random priors lack semantic information, which limits their effectiveness. 
This approach has remained unexplored in existing data-free UAP methods, as random priors lack semantic information, limiting its effectiveness.
In contrast, our pseudo-semantic prior contains richer semantic content than random priors, enabling improved transferability to unknown models through input transformations.
%enabling our method to achieve better transferability to unknown models through input transformations.
% We also incorporate input transformations into our data-free UAP framework to enhance transferability across models, a technique widely used in image-specific adversarial attacks. 
% This technique is less explored in data-free UAPs since a random prior has limited effectiveness ue to its lack of semantic information.
% In contrast, our pseudo-semantic prior contains more meaningful semantic content than a random prior, allowing our method to achieve improved attack transferability to unknown models through input transformations.
% While input transformations are less explored in data-free UAPs due to the use of random priors, which lack semantic information, our method effectively leverages them, as our pseudo-semantic prior contains diverse information, leading to improved performance in black-box settings.
% \chany{A random prior has limited effectiveness with input transformations due to its lack of semantic information.
% In contrast, our pseudo-semantic prior contains more meaningful content than a random prior.
% The semantic information in pseudo-semantic priors allows our method to achieve improved attack transferability to unknown models through input transformations.
% }


% In this paper, we propose a novel data-free UAP method called PSP-UAP which employs pseudo-semantic prior crafted from UAP and simple random noise to reduce the limitations of data-free constraints for training UAP. 
%In particular, UAPs tend to have a dominant label, and this is also true for UAPs in the optimizing stage.
% Additionally, maximizing the activation of convolutional layers crafts the most typical and robust patterns of the pre-trained surrogate model.
% These patterns are capable of deceiving the target model despite their imperceptible magnitude.
% This insight indicates that the UAP contains diverse and robust semantic information against any input images though not guaranteed to result in a dominant label.
% Hence, we randomly crop and resize portions of the UAP during training to create surrogate data samples, which we call pseudo-semantic priors. 
% This allows for the use of more diverse activated regions and various semantic information to deceive the model more effectively despite lacking the prior dataset.
% On the other hand, the randomly cropped, resized, and replaced pseudo-semantic priors inevitably vary in quality as training data.
% Averaging the activations of these samples equally disrupts the generation of an optimal UAP.
% To address this, we introduce an activation re-weighting loss to account for these differences.
% Finally, to maximize the utility of the generated pseudo-semantic priors, we incorporate input transformation attack methods to enhance attack transferability.

% However, the adversary does not always know the target data domain, so data-free universal attacks generated from random noise have recently been attracted.
% Conventional data-free universal attacks exhibit constrained transferability as they rely on random noise without any prior knowledge of the image dataset


\iffalse
Prior works have investigated various adversarial attack methods to craft AEs that can transfer to different deep neural networks (DNNs).
For example, FGSM and Deepfool~\cite{FGSM, Deepfool} generate AEs to fool target models, while MI-FGSM and CFM~\cite{mifgsm, clean_feature} aim to craft transferable AEs that can transfer across black-box DNN models.
%However, these methods can only generate perturbations for specific images, which cannot be generalized to attack other unknown images.
However, these methods generate unique perturbations for each specific image, which is inadequate for effective generalization to other images.
In contrast to these image-specific attacks, UAP~\cite{UAP} proposed a universal adversarial attack that generates a single image-agnostic perturbation capable of misleading a wide range of unknown images.
%The universal adversarial perturbation (UAP) is typically trained on prior samples from the target domain, enabling the generated UAP to effectively attack datasets that are similar to the prior.
%Universal adversarial attack methods generate a single perturbation from the entire target dataset, trained to disrupt predictions for most images within a similar domain.
%However, adversaries do not always have access to target domain samples, making data-free UAPs more practical and challenging, as they do not rely on any data from the target domain.
Although UAP degrades diverse images with a single perturbation, it still requires data samples from the target domain.
In some cases, however, adversaries lack access to data prior to the target domain, underscoring the need for data-free UAP methods.
Generating data-free UAP presents a more challenging problem than conventional UAP generation tasks, as it restricts the use of any prior knowledge of the target domain dataset.
Instead, previous works attempt to craft UAP at the feature level of convolutional neural networks (CNNs) by either maximizing~\cite{FFF, gd-uap, TRM} or disrupting~\cite{pd-ua, AAA} the activation of convolutional layers.
However, current data-free UAPs focus on leveraging the activations of the surrogate model's convolutional layers, leading to limited transferability to black-box models.


%-------------------------------------------------------------------------

%In that sense, a data-free UAP, which does not require any target domain prior, reduces the effort and cost associated with obtaining target domain data, making it a more efficient and realistic task.
%Unlike data-dependent UAP approaches, which guarantee semantic information and maximize cross-entropy, data-free UAPs cannot access to semantic information.

%-------------------------------------------------------------------------

In this paper, we propose a novel data-free UAP method called PSP-UAP which employs pseudo-semantic prior crafted from UAP and simple random noise to reduce the limitations of data-free constraints for training UAP. 
%In particular, UAPs tend to have a dominant label, and this is also true for UAPs in the optimizing stage.
Additionally, maximizing the activation of convolutional layers crafts the most typical and robust patterns of the pre-trained surrogate model.
These patterns are capable of deceiving the target model despite their imperceptible magnitude.
This insight indicates that the UAP contains diverse and robust semantic information against any input images though not guaranteed to result in a dominant label.
Hence, we randomly crop and resize portions of the UAP during training to create surrogate data samples, which we call pseudo-semantic priors. 
This allows for the use of more diverse activated regions and various semantic information to deceive the model more effectively despite lacking the prior dataset.
On the other hand, the randomly cropped, resized, and replaced pseudo-semantic priors inevitably vary in quality as training data.
Averaging the activations of these samples equally disrupts the generation of an optimal UAP.
To address this, we introduce an activation re-weighting loss to account for these differences.
Finally, to maximize the utility of the generated pseudo-semantic priors, we incorporate input transformation attack methods to enhance attack transferability.
\fi 

The main contributions can be summarized as follows:
\begin{itemize}
    \item We propose PSP-UAP, a novel data-free universal attack method that generates {{pseudo-semantic priors}} from the UAP itself, using inherent semantic information of the UAP as an alternative data source during training.
    \item 
    Our sample reweighting method prioritizes challenging examples during UAP training, minimizing the influence of uninformative samples that arise from random sampling within our pseudo-semantic prior.
    % Our sample reweighting method effectively focuses on challenging examples during UAP training, reducing the impact of uninformative samples arising from random sampling within our pseudo-semantic prior.
    \item We are the first to incorporate input transformations into the data-free UAP framework by leveraging pseudo-semantic priors with diverse semantic cues, boosting transferability across various CNN architectures in black-box settings.
    % \item We adopt input transformations commonly used in image-specific adversarial attacks to the data-free UAP framework, boosting transferability across different CNN architectures, especially in black-box settings.
    \item Our method achieves outstanding performance over the state-of-the-art data-free UAP methods by a substantial margin, and even outperforms existing data-dependent UAP methods.
\end{itemize}


\iffalse
\begin{itemize}
    %\item We propose a novel data-free universal attack that identifies and implements a method to leverage semantic information, overcoming the limitations of the data-free setting by maximizing its use even in the absence of data.
    \item We propose a novel data-free universal attack method that explores the semantic information of UAP by leveraging the properties of UAP to generate diverse pseudo-semantic priors, thereby overcoming the limitations of the data-free setting by fully utilizing available semantic cues even in the absence of data.
    \item {Since each generated pseudo-semantic prior can be viewed as an image with diverse semantics, our method can be integrated with various input transformation attack techniques applied to these pseudo-semantic priors. This is a key feature of our method.}
    \item We design an uncertainty-based re-weighting function to improve the utility of universal attacks using generated pseudo-semantic priors, enabling the UAP to train more intensively on certain semantic priors.
    \item {Extensive experiments demonstrate that our PSP-UAP has superior performance compared with other data-free UAP methods.}
\end{itemize}
\fi



==> sec/3_method.tex <==


\section{Methodology}

In this section, we present our motivation and approach for generating the pseudo-semantic prior. 
We then describe our sample reweighting strategy for optimizing UAP, followed by input transformations applied to semantic samples derived from the pseudo-semantic prior.
% In this section, we present the motivation and our approach for generating a pseudo-semantic prior.
% And then, we describe the use of sample reweighting to create an optimal UAP, along with the application of input transformation to the semantic samples drawn from the pseudo-semantic prior.
%In this section, we present the motivation for creating and augmenting priors with semantic information. Then, we propose methods for augmenting these priors and applying weighted emphasis while optimizing UAP.



\subsection{Preliminaries of data-free UAP}

Universal adversarial attacks aim to optimize a single perturbation $\delta$ using a model $f$ that effectively deceives most of the samples $I$ in the target domain dataset, with the pixel intensities of $\delta$ restricted by a constraint parameter $\epsilon$:
%\jeany{This sentence is not grammatically correct.}, as follows:
\begin{align}
    f (I + \delta) \neq f (I), \text{~~~s.t.~~} \| \delta \|_{\infty} \leq \epsilon.
    \label{eq:obj}
\end{align}
%In a data-free setting, we cannot access the target domain dataset while generating UAP.
%Exploiting target domain data to create UAPs that disrupt patterns in real images is an intuitive and reasonable approach.
However, in data-free settings where the target dataset is inaccessible, UAPs are typically trained using simple random priors, such as Gaussian noises or jigsaw images~\cite{cosine, TRM}.
% Given these random priors~$p_{z}$, the previous data-free UAP work, such as GD-UAP~\cite{gd-uap}, introduced an activation maximizing loss as follows:
Given these random priors~$p_{z}$, GD-UAP~\cite{gd-uap} introduced an activation maximizing loss as follows:
%To solve this problem, FFF~\cite{FFF} propose to maximize the CNN activations:
% Representative data-free UAP approach,
%\begin{equation}
%\begin{aligned}
%    \underset{v}{\text{max}} \quad &\|\mathcal{A}_{i} \|_{2}, \quad \text{for} \ i=1,2,\cdots,L \\
%    &\text{s.t.} \quad \|v\|_{\infty} \leq \epsilon
%\end{aligned}
%\label{eq:objective}
%\end{equation}
\begin{gather}
    %\mathcal{L} = -\sum_{\mathbf{x}^r\sim N(\mu,\sigma)}\sum_i^N{\log{\|\mathcal{A}_{i}(\mathbf{x}^r+ \delta)}\|_2},
    %\mathcal{L} = -\sum_{{z}\sim \mathbf{Z}}\sum_i^L{\log{\|\mathcal{A}_{i}({z}+ \delta)}\|_2},\label{eq:GDUAP}\\
    \mathcal{L} = -\mathbb{E}_{{z}\sim p_{{z}}}\sum_{i=1}^L{\log{\|\mathcal{A}^f_{i}({z}+ \delta)}\|_2},\label{eq:GDUAP}\\
    \text{s.t.~~} \| \delta \|_{\infty} \leq \epsilon \nonumber, 
\end{gather}
where $\mathcal{A}^f_{i}(\cdot)$ indicates the activation of the $i$-th layer of the surrogate network $f$, $L$ denotes the number of layers in $f$, and ${z}$ represents pseudo-data sampled from a simple random prior distribution, $p_{{z}}$.
%UAP, $\delta$ is optimized to maximize the activation by minimizing this objective function.
%Since the target pre-trained model does not undergo further training when crafting the UAP, it dominates the image with a low intensity, forming a pattern that is both dominant and typical~\cite{dominant, cosine} to fool target model.
This loss is designed to overactivate features extracted from multiple convolutional layers of the surrogate model without input images.
Consequently, the distorted activation interferes with feature extraction, leading CNN models to make incorrect predictions~\cite{FFF, gd-uap}.
% The contaminated activation distorts feature processing, resulting in misclassification by CNN models~\cite{FFF, gd-uap}.% 
% \jeany{$\leftarrow$ What does this mean?}
%Since UAPs need to dominate all perturbed data when input into the target model, they form dominant patterns~\cite{cosine}. \jeany{$\leftarrow$ What does this mean?}




\subsection{Pseudo-Semantic Prior} 

%In data-free methods, however, UAP is generated from random simple priors such as Gaussian noises or artificial jigsaw puzzles, and the absence of semantic information in these priors does not adequately ensure sufficient degradation of the semantic content in real images.
%UAPs are generated from simple random noises in a data-free setting.
Although data-free UAP methods~\cite{gd-uap, TRM} use random priors, such as Gaussian noises or artificial jigsaw puzzles, to mimic the statistical properties of image datasets, they are still limited by a lack of semantic information.
Furthermore, since UAPs are trained by maximizing activations in network layers, they tend to overfit to surrogate models.  
Optimizing UAPs without semantic content and relying on  activation or outputs of surrogate networks, reduces their effectiveness in disrupting real images in unseen models, leading to degraded performances in black box transferability.
% As a result, UAPs generated by data-free UAP methods tend to perform worse especially in white box attacks than those generated by data-dependent methods, where data priors are accessible.

% This lack of semantic information in such noises limits their ability to effectively disrupt the semantic content of real images.
% As a result, UAPs generated by data-free methods tend to poorly perform in black-box attacks and show weak transferability to other models, 
%as they primarily capture the dominant patterns of the surrogate model~\cite{cosine}.
%as they primarily capture the dominant patterns of the surrogate model 이 부분이 적절하지 않은 것 같아서 바꿨습니다. OK
% \chany{GD-UAP~\cite{gd-uap} enhanced the attack performance by adding random priors that mimic the statistical properties of image datasets to UAP during optimizing.
% These random priors, however, fail to capture the patterns inherent in real images.
% As a result, UAPs generated by data-free methods tend to perform poorly in black-box attacks, due to the lack of semantic information in the random priors.
% }

%To address this issue, we propose a method that augments the prior using UAP, ensuring that the prior contains comprehensive semantic information.

To address these issues, we aim to enhance the semantic content within a data-free UAP framework, inspired by previous works~\cite{UAP, sga-uap, cosine, TRM} that demonstrate the presence of dominant labels in generated UAPs.
For instance, early works~\cite{UAP, sga-uap} observed that untargeted UAPs often cause misclassification toward a dominant label, a property that also holds in data-free settings~\cite{TRM}.
Cosine-UAP~\cite{cosine} further showed that the logit distribution of UAPs tends to dominate that of the input data $x$.
This suggests that, although the UAP is a subtle perturbation, it behaves like a single image with strong semantic information, guiding the model toward classification with a dominant label.
% This implies that, despite being a subtle perturbation, the UAP acts as a single image containing strong semantic information that leads to classification toward a dominant label.

Inspired by this observation, we leverage the inherent semantic information in UAPs by treating the combination of UAP and random noise as a single image, termed the \textbf{\textit{pseudo-semantic prior}}, to resolve the lack of semantic content in data-free UAP training.
As shown in Figure~\ref{fig:fig_1} and Figure~\ref{fig:fig_3}, the generated UAPs exhibit diverse semantic labels across different regions.
Although {regions within the UAP are} classified under the same label, the attention heatmaps generated by Grad-CAM~\cite{gradcam} show distinct patterns, suggesting that diverse semantic patterns are embedded within the UAP.
% Regions within the UAP show the attention heatmaps generated by Grad-CAM~\cite{gradcam} with distinct patterns from the original UAP, suggesting that diverse semantic information is embedded within the UAP.
% Although {regions within the UAP are} classified under the same label, the attention heatmaps generated by Grad-CAM~\cite{gradcam} show distinct patterns, suggesting that diverse semantic information is embedded within the UAP.
% Even when classified under the same label, the attention heatmaps generated by Grad-CAM~\cite{gradcam} show distinct patterns, suggesting that a variety of semantic information is embedded within the UAP.
% In addition, even with the same label, the attention heatmaps obtained by Grad-CAM~\cite{gradcam} appear differently, indicating that diverse semantic information is embedded within the UAP.
% When viewing an image in its entirety, we integrate all available information to recognize a single label.
% However, if only a specific image region is considered, it may be interpreted as a different label as shown in Figure~\ref{fig:fig_1}. 
% This phenomenon is also observed in UAP, as shown in Figure~\ref{fig:fig_3}. 
% Furthermore, even with the same label, the attention heatmaps obtained by Grad-CAM~\cite{gradcam} appear differently, indicating that diverse semantic information is embedded within the UAP.
% This finding also motivates us to explore ways to leverage this pseudo-semantic prior's potential fully.
% we leverage the inherent semantic information within UAP by treating the sum of UAP and random noises as a single image, which we call \textit{pseudo-semantic prior}.
% the prior with UAPs can be treated similarly to an image, allowing for data augmentation using techniques analogous to those employed in image augmentation.


%even sub-parts of the image, which are cropped and resized back to the original size, are predicted to different labels.
%This observation motivates us to explore ways to leverage the abundant semantic information of UAP on optimizing stage.
Building on the above insight, we generate pseudo-data samples from the pseudo-semantic prior to enrich the semantic content, which we refer to as \textbf{\textit{semantic samples}} $x_n$:
% We generate the semantic samples from the pseudo-semantic prior as follows:
\begin{gather}
    \mathbf{x} \sim p_{\mathbf{x}|p_{{z}}, \delta_t} = \{{z} + \delta_t \vert  {z} \in p_{{z}}\}, \label{SP} \\
    \{{x}_1, {x}_2, ..., {x}_N\} = \mathcal{C}(\mathbf{x}; N),
    \label{crop_resize}
    %&\mathbf{x}^{(n)} = \mathcal{C}(\mathbf{x}; N), \\
    %&\mathbf{X} = \{x_1, x_2, ..., x_N\} = \mathcal{C}(\mathbf{x}; N), , \\
    %&{X} = \{{x}^{(1)}, x^{(2)}, ..., x^{(N)}\} = \mathcal{C}(\mathbf{x}; N),\\
    % \mathbf{x} \sim p_{\mathbf{x}|p_{{z}}, \delta_t} = \{\mathcal{C}({z} + \delta_t) \vert  {z} \sim p_{{z}}\},
    % \mathbf{x} &\sim p_{\mathbf{x}|p_{{z}}, \delta_t},
    % p_{\mathbf{x}}(p_{{z}}, \delta_t) &= \{\mathcal{C}({z} + \delta_t) \vert  {z} \sim p_{{z}}\},\\
    % \mathbf{x} &\sim p_{\mathbf{x}}(p_{{z}}, \delta_t),
    % \\
    % \mathbf{x}^r &\sim \mathbf{p}_r, \\
    %\mathbf{p}_s &= \mathbf{x}^r + \text{SG}(\delta_t), \\
    %\mathbf{x}^s &\sim \mathbf{p}_s, \\
    %p_{{x}}({z}, \delta_t) &= {z} + \text{sg}(\delta_t), \text{  } {z} \sim p_{{z}}\\
    %\mathbf{x}^s &\sim \text{Sample}(\mathbf{x}^r,\text{SG}(\delta_t)), \\
    %\mathbf{x}^\mathbf{T} &= \mathbf{T}(\mathbf{x} + \delta_t),
    %\mathbf{x}^s &= S(\mathbf{p}_t),
    %\label{eq:crop_resize}
\end{gather}
where ${z}$ and $\delta_t$ denote random noise sampled from $p_{{z}}$ and the UAP being trained in $t$-th iteration, respectively.
% The semantic prior $p_{{x}}$ is obtained by summing ${z}$ and $\delta_t$, where the gradient of $\delta_t$ is stopped.
The pseudo-semantic prior $p_{\mathbf{x}}$ denotes a set of adversarial examples with $\delta_t$ derived from the random prior distribution.
$\mathcal{C}$ is a sampler that draws $N$ numbers of semantic samples ${x}_n$ from $p_{\mathbf{x}}$ by applying crop and resize operations.
Specifically, we randomly crop a region of the UAP, and resize it to the original scale of the UAP size.
We believe that leveraging the generated semantic information embedded in different regions of the UAP provides more effective guidance for successfully attacking target features than relying solely on random noise.
% We believe that, given the learned semantic information in UAP, semantic samples provide more effective semantic guidance on target features than random noise.
% We randomly crop a region of the UAP, then resize it to random scale of the original UAP size, padding with the original pixel values from the pseudo-semantic prior.
% We randomly crop a region and resize it to the original UAP size 
% The cropping and resizing are performed with a random scale and aspect ratio.
%and each cropped and resized sample is positioned at a random location.
% To prevent loss of semantic information, the remaining areas after resizing and replacing are filled with the original pixel values from the pseudo-semantic prior.
%obtained from $p_{\mathbf{x}}$ contains the recognizable patterns of the model imitated by the UAP.

%Note that $\mathbf{x}$ is randomly cropped during sampling to prevent overlapping patterns with the UAP $\delta_t$ being trained.
%After that, Sampler($\cdot$) randomly crops and resizes the abundant content located in various parts of the semantic prior to sample $N$ pseudo-data.
%Note that the $\delta_t$ is added to $\mathbf{x}$ before passing the sampler since $\mathbf{x}+\delta_t$ is treated as a single image.

% Through this motivation and process, we generate semantic samples with diverse content that are regarded as data, all within a data-free constraint.

% crop resize 등등 서술
%Since the semantic prior is regarded as a single image, we create pseudo training data samples through data augmentation, applying techniques similar to those used in image processing as following:




\subsection{Sample Reweighting}
Semantic samples are randomly drawn from the pseudo-semantic prior, leading to an imbalance in difficulty due to variations in semantic content; some samples are easily fooled by the UAP, while others are more difficult to deceive.
% Treating these samples equally may hinder optimal UAP updates.
To tackle this, we propose a new sample reweighting method that prioritizes harder-to-fool samples. 

Specifically, we compute the weight of each sample using the KL divergence between the original input and its adversarial counterpart during training. 
% We define the posterior~$P$ and approximated distribution~$Q$ from each semantic sample and adversarial example of the semantic sample using the current UAP, respectively, as follows:
We define the original distribution~$P$ and the adversarial distribution~$Q$ from each semantic sample and its corresponding adversarial example generated by the current UAP, respectively, as follows:
\begin{align}
    &P({x}_n) = f({x}_n) \label{eq:ppp},\\
    &Q({x}_n) = f({x}_n+\delta_t) \label{eq:qqq},
\end{align}
where $f(\cdot)$ is the temperature-scaled softmax output of a surrogate model.
% $N$ indicates the number of $\mathbf{x}$ sampled from the semantic prior $p_{\mathbf{x}}$, 
%The distribution of $\mathbf{x}$ is designated as the posterior and $\mathbf{x}+\delta_t$ as the approximate posterior.
Then, we calculate the weights of each semantic sample using the KL-divergence:% where $\text{w}_j \in \mathbf{w}$.
\begin{align}
    &w_n = D_{KL}(P({x}_n)\|Q({x}_n))^{-1}.
    \label{eq:weight_1}
\end{align}
The large KL-divergence value indicates that $\delta_t$ has significantly altered the distribution of ${x}_n$, whereas a small value suggests an ineffective attack.
Thus, we take the reciprocal of KL-divergence values to assign greater weights to semantic samples where the attack results in minimal distributional change.
We reweight the semantic samples using the weights generated from Eq.~\eqref{eq:weight_1}, considering the influence of the UAP on each sampled ${x}_n$, which enables us to optimize the UAP effectively.
%taking into account the influence of the UAP on each sampled $\mathbf{x}$, allowing us to find optimal UAP.


\iffalse
Training with semantic samples is more effective than with random noise for generating UAPs, as semantic samples contain more meaningful information.
%However, some pseudo-semantic priors have already been learned by the UAP, using all of them equally in training may hinder the generation of an optimal UAP and lead to overfit.
However, directly averaging activations across all samples hinders the optimal UAP update. 
%Pseudo-semantic samples are randomly cropped from the semantic prior, so their activations may result in an imbalance of semantic information.
Semantic samples are randomly sampled from the pseudo-semantic prior, so they have imbalanced semantic information.
%The basic loss function Eq.~\eqref{eq:GDUAP} is designed to excessively activate features extracted from multiple convolutional layers of surrogate model regardless of the input image.
%This leads to the accumulation of unnecessary and contaminated activations, which induces ambiguous predictions~\cite{FFF, gd-uap}.
%Also, DF-UAP~\cite{mutual} suggests an interpretation that UAPs are features while training data samples behave like noise to them.
%Thus, it is unreasonable to treat pseudo-semantic samples that become ambiguous after adding the UAP the same as those that still retain discriminating predictions.
This leads to a disparity between samples that satisfy Eq.~\eqref{eq:obj} and those that do not follow. 
%Therefore, it is not appropriate to treat these samples equivalently during UAP training.
%Suppose the training data for learning the UAP consists only of random Gaussian noise and an image with a specific label.
To maximize the use of $p_{\mathbf{x}}$, we reformulate the weight of each sample by designing a reweighting method based on KL divergence.
\fi

%According to Eq.~\eqref{eq:obj}, the objective of a universal attack is to lead predictions to a label different from the original prediction label.
%Data-free universal attacks cannot utilize any information related to class labels.
%Therefore, we assess the success of the attack based on the uncertainty when a semantic prior is attacked by the UAP, assigning higher weights to the activation of semantic priors with lower uncertainty, using the inverse of entropy as the weight as follows:
%However, directly applying the weights generated by Eq.~\eqref{eq:weight_1} is not suitable because the entropy distribution of logits does not follow any specific distribution. 

%Consequently, overly large weights may be assigned to certain pseudo-semantic samples, potentially exerting a dominant influence on UAP training.
%Also, this could lead to the disregard of information from semantic priors with higher entropy, as they receive relatively lower weights.
%To address this, we apply the softmax function to smooth the weights as shown in Eq.~\eqref{eq:weight_2}, where $\tau$ is the temperature parameter, dynamically adjusted to account for variations in logit distributions across different models.
%This ensures that the softmax output can be appropriately calibrated for each model's specific logit characteristics.

%s a result, larger weights remain relatively higher without weight exploding, while smaller weights are prevented from becoming so diminished that they are effectively disregarded in comparison to larger weights.


%Input transform 들어가기 전에 pseudo code 추가

\subsection{Input Transformation}
To enhance black-box attack transferability, we incorporate input transformation techniques into our semantic samples. 
While input transformation is commonly used in image-specific adversarial attacks, it has been less explored in data-free UAPs due to the limited semantic information in random priors. 
In our method, however, the semantic samples generated from pseudo-semantic priors contain diverse semantic cues, making input transformations more effective in a data-free setting.


% To improve the black-box attack transferability, we adapt the input transformation attack methods to our semantic samples.
% Input transformation is widely used in image-specific adversarial attacks but less explored in data-free UAPs, due to the lack of semantic information in random prior.
% In our method, since semantic samples generated by pseudo-semantic priors contain diverse semantic information,  make use of input tranformation more effectively.

Following L2T~\cite{L2T}, which shows that rotation, scaling, and shuffling are particularly effective for improving attack transferability, we randomly select one of these transformations and apply it to each semantic sample.
% $T(\cdot)$
% Following L2T~\cite{L2T} showing that among various transformations, rotation, scaling, and shuffling are effective in improving attack transferability, we randomly select a transformation $T(\cdot)$ from these three transformations and apply it to each semantic sample.
For rotation, the angle $\alpha$ is drawn from a truncated normal distribution within the range $-\theta \leq \alpha \leq \theta$.
Scaling is applied with a uniform distribution within the bounds $\beta_{low} \leq \beta \leq \beta_{high}$.
Shuffling involves randomly rearranging $m\times m$ blocks.
During optimization, applying input transformations to our PSP-UAP increases the variation of semantic samples and enhances the black-box attack transferability.

\iffalse
% optimize 전략인 curriculum과 p_rate를 사용한 거를 여기에 적어야겠지? input transformation도 내가 처음 제시하는 게 아니고, 앞에 둘도 TRM에서 제시한 거니까 여기 마지막에 한번에 설명
To improve the black-box attack transferability, we apply the input transformation attack methods to our semantic samples derived from pseudo-semantic prior.
% It is not surprising that applying transformations to data samples for adversarial attack,but this is the first attempt in data-free universal attack since we create pseudo-semantic samples that can serve as data.
L2T~\cite{L2T} shows that among various transformations, rotation, scaling, and shuffling are effective in improving attack transferability.  
%Inspired by this, we randomly apply these three transformations to the pseudo-semantic samples.
%The overall loss function of our PSP-UAP is as follows:
%\begin{gather}
    %\mathcal{L} = -\sum_{\mathbf{x}^r\sim N(\mu,\sigma)}\sum_i^N{\log{\|\mathcal{A}_{i}(\mathbf{x}^r+ \delta)}\|_2},
    %\mathcal{L} = -\sum_{\mathbf{x}\sim p_{\mathbf{x}}(p_{{z}},\delta_t)}\sum_i^{l'}{\log{\text{w}_j \|\mathcal{A}_{i}(T(\mathbf{x}+ \delta))}\|_2},
    %\mathcal{L} = -\mathbb{E}_{\mathbf{x} \sim p_{\mathbf{x}}} \sum_{n}^N \sum_{i}^L{\log{\text{w} %\|\mathcal{A}_{i}(T(\mathbf{x}^{(n)}+ \delta_t))}\|_2},
    % \mathcal{L} = -\mathbb{E}_{\mathbf{x} \sim p_{\mathbf{x}}}\sum_{i}^L{\log{\text{w} \|\mathcal{A}_{i}(T(\mathbf{x}+ \delta_t))}\|_2},
    %\nonumber \mathbf{x}_j \sim p_{\mathbf{x}}(p_{{z}},\delta_t),
%    \label{eq:reweight and transform}
%\end{gather}
% \begin{equation}
% \begin{aligned}
%     %\mathcal{L} = -\sum_{\mathbf{x}^r\sim N(\mu,\sigma)}\sum_i^N{\log{\|\mathcal{A}_{i}(\mathbf{x}^r+ \delta)}\|_2},
%     \mathcal{L} = -\frac{1}{\left|N\right|}\sum^N_{\mathbf{x}^s_j\sim \mathbf{p}_s}\sum_i^{l'}{\log{\text{w}_j \|\mathcal{A}_{i}(T(\mathbf{x}^s_j+ \delta))}\|_2},
% \end{aligned}
% \label{eq:reweight and transform}
% \end{equation}
Inspired by this, we randomly select a transformation $T(\cdot)$ from these three transformations and apply it to each semantic sample.
For rotation, the angle $\alpha$ is drawn from a truncated normal distribution within the range $-\theta \leq \alpha \leq \theta$.
Scaling is applied with a uniform distribution within the bounds $\beta_{low} \leq \beta \leq \beta_{high}$.
Shuffling involves randomly rearranging $m\times m$ blocks.
During the optimization process, input transformation attack methods increase the variance\chany{variation} of semantic samples and lead to enhancing the black-box attack transferability for our PSP-UAP.
\fi


%Moreover, the KL re-weighted loss assigns greater weight to pseudo-semantic samples whose probability distribution changes minimally even after adding the UAP.
%The entire PSP-UAP algorithm is summarized in Algorithm~\ref{alg:psp-uap}.


\input{table/algorithm}




\subsection{Overall Loss}
We integrate the pseudo-semantic prior, sample reweighting, and input transformation into Eq.~\eqref{eq:GDUAP} to optimize the proposed PSP-UAP.
The final loss function of our PSP-UAP is defined as follows:
\begin{gather}
   \mathcal{L} = -\mathbb{E}_{\mathbf{x} \sim p_{\mathbf{x}}} \sum_{n=1}^N \sum_{i=1}^{l}{\log{(w_n \|\mathcal{A}^f_{i}(T({x}_n+ \delta_t))}\|_2)},
    \label{eq:overall loss}
\end{gather}
where $\mathcal{A}^f_{i}(\cdot)$ denotes the activation of the $i$-th layer in network $f$, ${x}_n$ represent the $n$-th semantic sample extracted from the pseudo-semantic prior $p_{\mathbf{x}}$, $\delta_t$ denotes the UAP at the $t$-th iteration,
$w_n$ is the weight of ${x}_n$ from Eq.~\eqref{eq:weight_1}, $l$ indicates the number of the convolutional layers used in the activation sum,
$T(\cdot)$ denotes a randomly selected transform for input transformation, and $N$ is the number of semantic samples extracted from one pseudo-semantic prior.

% Note that Eq.\eqref{eq:ppp} and Eq.~\eqref{eq:qqq} are computed after applying $T(\cdot)$ to both the semantic sample and its adversarial example.
% Optimizing the overall loss, we take full advantage of the generated semantic samples as data to generate a highly transferable UAP even in the absence of prior knowledge of the target domain.

By optimizing the overall loss, we fully leverage the generated semantic samples as data to produce a highly transferable UAP, even without prior knowledge of the target domain. 
The overall PSP-UAP framework and detailed algorithm are shown in Figure~\ref{fig:framework} and Algorithm~\ref{alg:psp-uap}, respectively.


\begin{figure}[t]
\centering
    \includegraphics[width=\linewidth]{figures/fig_3_1.pdf}
    \caption{
    Semantic samples derived from an adversarial example during training, along with their predicted labels and GradCAM heatmaps from Dense-121. 
    Despite originating from the same example, the variations in predicted labels and heatmaps indicate that these semantic samples capture diverse semantic features. %, suggesting that the UAPs are trained to effectively deceive the model without any data.
    % Pseudo-semantic samples extracted from the pseudo-adversarial example during training, along with their attention heatmaps using GradCAM and predicted labels generated by Dense-121, are shown. The leftmost column presents the original UAP, while the next three columns display pseudo-semantic samples cropped from color-matched regions. Although these samples are derived from the same UAP, their predicted labels and heatmaps differ. This implies that the pseudo-semantic samples capture diverse semantic features within the same UAP, highlighting its ability to generate varied representations that can effectively deceive the model in multiple ways without any data.
    }
    \label{fig:fig_3}
\end{figure}

\input{table/white_box}


==> sec/4_Experiments.tex <==
\input{table/black_box_alex}
\input{table/black_box}
\input{table/data-dependent}


\section{Experiments}
\paragraph{Experimental Setup.} 
We follow the experiment setup in existing data-free universal attacks~\cite{gd-uap, TRM} to evaluate the performance of our PSP-UAP.
We evaluate the proposed method on ImageNet~\cite{Imagenet} validation set with five  ImageNet pre-trained CNN models, AlexNet~\cite{alex}, VGG16~\cite{vgg}, VGG19~\cite{vgg}, ResNet152 (RN152)~\cite{res152}, and GoogleNet~\cite{google}, which are commonly used in data-free UAP methods.
We further explore four additional CNN models including DenseNet121~\cite{dense}, MobileNet-v3-Large~\cite{mobile}, ResNet50~\cite{res152}, and Inception-v3~\cite{inception}, pre-trained on ImageNet dataset.

% We further explore four advanced CNN models including DenseNet121 (DN121)~\cite{dense}, MobileNet-v3-Large (MN-v3-L)~\cite{mobile}, ResNet50 (RN50)~\cite{res152}, and Inception-v3 (Inc-v3)~\cite{inception}, which are also pretrained using ImageNet dataset.

\paragraph{Evaluation Metrics.} To effectively evaluate the attack performance of our proposed method, we use the fooling rate $(FR)$ which is widely used in universal attacks ~\cite{UAP, TRM}.
$FR$ indicates the proportion of samples with label changes when applying UAP.

\paragraph{Baselines.} The proposed method is compared with the following data-free universal attacks, including FFF~\cite{FFF}, GD-UAP~\cite{gd-uap}, PD-UA~\cite{pd-ua}, Cosine-UAP~\cite{cosine}, AT-UAP~\cite{at-uap}, and TRM-UAP~\cite{TRM}.
Since AT-UAP includes both data-free (AT-UAP-U) and data-dependent (AT-UAP-S) versions, we evaluate both in our experiments.
% AT-UAP has both data-free (AT-UAP-U) and data-dependent (AT-UAP-S) versions and we compare them both in our experiments.
We also compared our method with SGA-UAP~\cite{sga-uap} which is one of the state-of-the-art data-dependent universal attacks.
%For a fair comparison, GD-UAP~\cite{gd-uap} and TRM-UAP~\cite{TRM} are reproduced by making the setup consistent with our method.

\vspace{-0.2cm}
\paragraph{Implementation Details.} Our experiments are implemented on PyTorch with a single NVIDIA A6000 GPU.
We set $\epsilon$ $=$ $10/255$ to restrict $\ell_{\infty}$-norm, the maximum iteration $T$ as $10,000$, and the saturation threshold $r$ to $0.001\%$, following the setting in TRM-UAP~\cite{gd-uap, TRM}.
For input transformations, we set $\theta$ $=$ $6$ for rotation, $\beta_{low}$ $=$ $0.8$ and $\beta_{high}$ $=$ $4$ for scaling, and $m$ $=$ $2$ for random shuffling.
Moreover, the number of semantic samples $N$ is set to $10$.
We define temperature parameter $\tau \in \{1.0, 5.0, 5.0, 3.0, 5.0\}$ corresponding to AlexNet, VGG16, VGG19, ResNet152, GoogleNet.
For the additional CNN models, we set $\tau \in \{3.0, 10.0, 2.0, 3.0\}$ corresponding to ResNet50, DenseNet121, MobileNet-v3-Large, Inception-v3.
We follow the same curriculum learning and saturation check strategy of TRM-UAP.
We set different ratios to use the activation of intermediate layers across different models.
To ensure a fair evaluation, we find the optimal parameters for TRM-UAP on RN50, DN121, MB-v3-L, and Inc-v3 through our best efforts.

%---------------------------------------------------------------------%


\subsection{Evaluation on White-Box Attack}
We first evaluate UAPs generated by our PSP-UAP on various CNN models under the white-box setting.
We compare the attack performance of our UAPs with other data-free universal attacks on the ImageNet validation set, as shown in Table~\ref{tab:white_box}.
%We first generate UAPs on various CNN models under the white-box setting to evaluate the attack performance of our PSP-UAP with other data-free universal attacks on the ImageNet validation set, as shown in Table~\ref{tab:white_box}.
%Compared to other universal attacks, PSP-UAP demonstrates an improvement in $FR$.
% The $FR$ on AlexNet and GoogleNet is slightly lower compared to other methods, but we surpass all universal attack methods in terms of average $FR$. 
While the $FR$ on AlexNet and GoogleNet is slightly lower than other methods, our approach achieves the highest average $FR$ across all universal attack methods.
%the highest average $FR$ across all universal attack methods.
%Cosine-UAP and TRM-UAP perform the higher $FR$ than PSP-UAP on GoogleNet, and slightly on AlexNet, but PSP-UAP achieves the highest average white-box $FR$ across all other models.
%In general, $FR$ increased by $1.7\sim3.3\% $, with an especially remarkable $15\%$ rise in $FR$ on ResNet152.
Notably, the improvement on ResNet152 is substantial, with a $12.5\%$ increase in the $FR$, 
demonstrating that our PSP-UAP performs exceptionally well, particularly on deeper and more complex CNN models.

%After first examining black-box attack transferability on the five models in Table.~\ref{tab:white_box}, we conduct further experiments by comparing transferability of PSP-UAP with TRM-UAP, the state-of-the-art data-free universal attack, on ResNet50, ResNet152, DenseNet121, MobileNet-v3-Large, and Inception-v3 to verify the superiority of PSP-UAP method on larger CNN models.
% 기존 모델 5개에 대한 것은 결과 뽑히면 추가


\subsection{Evaluation on Black-Box Attack}

\paragraph{Comparison with SoTA Data-free UAPs.}
%Note that both AT-UAP and TRM-UAP are data-free methods, while SGA-UAP is data-dependent universal attack. 
%As shown in Table~\ref{tab:black_box_combined}, PSP-UAP achieves a higher average $FR$ than other data-free attack methods across all models except GoogleNet.
%Notably, our method demonstrates superior transferability with an average $FR$ improvement of 2.8$\sim$13.4\% over other data-free methods.
%While in some cases the performance of PSP-UAP is slightly below that of TRM or AT-UAP, its average $FR$ remains the highest overall.
We evaluate the transferability of our UAPs on commonly used CNN models in the black-box scenario.
Table~\ref{tab:black_box_combined} represents the attack performance across different settings, with columns representing target models and rows indicating surrogate models to craft the UAPs. 
As shown in Table~\ref{tab:black_box_combined}, PSP-UAP achieves superior results than other data-free attack methods across most models, with performance comparable to, but slightly below, TRM-UAP on GoogleNet. 
Notably, in strictly black-box settings (excluding the white-box scenario where GoogleNet attacks itself), PSP-UAP achieves an average $FR$ of 70.1\% compared to TRM-UAP’s 69.6\%, demonstrating better transferability.
% PSP-UAP achieves a higher average $FR$ than other data-free attack methods across most models, with performance comparable to, but slightly below, TRM-UAP on GoogleNet. 
% As shown in Table~\ref{tab:black_box_combined}, PSP-UAP achieves a higher average $FR$ than other data-free attack methods across most models, with performance similar to but slightly below that of TRM-UAP on GoogleNet.
% Especially in 
% Notably, PSP-UAP demonstrates superior transferability, with a significant improvement in $FR$ across most experiments compared to other data-free methods.
%Notably, PSP-UAP demonstrates superior transferability, showing the average $FR$ improvement of 2.8$\sim$13.4\% over other data-free methods. 
%Furthermore, PSP-UAP demonstrates the highest attack performance overall across all experiments, with a significant margin compared to other methods.
% Furthermore, PSP-UAP demonstrates the highest overall attack performance, with a significant margin compared to other methods.
% Although in some experimental results the performances of PSP-UAP are slightly below those of TRM or AT-UAP, the average $FR$ ($FR$) is the highest.
% For UAPs generated with GoogleNet, the black-box $FR$s of TRM-UAP and our method are nearly similar, but the standard deviation across all models is considerably lower for our method.
% These results suggest that our PSP-UAP has better generalization performance.

\vspace{-0.2cm}
\paragraph{Extended Evaluation with Additional CNN Models.}
To further explore the effectiveness of the proposed PSP-UAP, we conduct additional experiments on widely used CNN models, including ResNet50, DenseNet121, MobileNet-v3-Large, and Inception-v3.
We compare the attack performance of PSP-UAP with TRM-UAP as shown in Table~\ref{tab:black_box_advance}.
Note that we limit the comparison to TRM-UAP since the public code for AT-UAP has not yet been released.
The results demonstrate that our PSP-UAP consistently outperforms TRM-UAP in terms of $FR$ with a substantial margin.
The substantial improvement demonstrates PSP-UAP's strong generalization across diverse CNN models, highlighting the robustness of our approach.
% demonstrates that PSP-UAP is more adept at generalizing across models, highlighting the consistent excellence of our method.
%achieving a higher average $FR$ margin than other data-free methods.
% PSP-UAP delivers overall performance surpassing TRM-UAP, with an average $FR$ margin that is 13$\sim$23\% higher. 
% These results exhibit the effectiveness of PSP-UAP, as it achieves significantly increased $FR$ across diverse CNN architectures. 


\vspace{-0.2cm}
\paragraph{Comparison with Data-dependent UAPs.}
%To challenge the conventional notion that the lack of prior knowledge of the target domain limits attack performance of UAPs, we also compare our method to data-dependent universal attacks in the black-box scenario.
To verify whether our method effectively alleviates the lack of prior knowledge, we compare our method to state-of-the-art data-dependent universal attacks in the black-box scenario.
%\chany{We aim to challenge the conventional notion that the lack of prior knowledge of the target domain limits the transferability of UAPs.
%To do so, we also compare our method to data-dependent universal attacks in the black-box scenario.}
As shown in Table~\ref{tab:black_box_data_dep}, the $FR$ of white-box attacks is inevitably higher for SGA-UAP and AT-UAP-S, as they fully utilize the target domain dataset.
%AT-UAP crafts certain UAPs that, when transferred from models like AlexNet, VGG16, or VGG19, achieve higher FR than SGA-UAP, but AT-UAP does not show generalized performance.
On the other hand, PSP-UAP exhibits superior transferability, as observed in the black-box setting.
Our method outperforms by achieving a higher average $FR$ across most models, surpassing data-dependent approaches.
Furthermore, even in cases where some $FR$ results are lower, they do not fall significantly behind the data-dependent universal methods.
%The UAP crafted on VGG19 shows only a minimal performance difference of less than 2\% when transferred to AlexNet and VGG16.
%and although the average $FR$ on GoogleNet is slightly lower, our method consistently outperforms other models.
These results indicate that our semantic samples prove to be effective as data for training the UAP, successfully overcoming the limitation posed by the absence of a target domain.

\begin{figure}[t]
\centering
    \includegraphics[width=1\linewidth]{figures/figure_6.pdf}
    \vspace{-0.6cm}
    \caption{Visualization of UAPs crafted by PSP-UAP during training on DenseNet121, ResNet152, and AlexNet. From left to right, the UAPs are shown at iterations 100, 900, 1700, and the final UAP after training. Pixel values are scaled to [0, 255].
  }
  \vspace{-0.1cm}
    \label{fig:uaps}
\end{figure}


\begin{figure}[t]
\centering
    \includegraphics[width=\linewidth]{figures/ablation.pdf}
    \caption{
    Ablation study on each proposed component in PSP-UAP.
    RP and PSP refer to training a UAP using random noises and semantic samples drawn from pseudo-semantic prior, respectively.
    RW and T denote the use of sample reweighting, and input transformation, respectively.
    % the pseudo-semantic prior, sample reweighting, and input transformation, respectively.
    % Random prior, pseudo-semantic prior, sample reweighting, and input transformation are denoted by RP, PSP, RW, and T, respectively.
    % SP, RW, and T denote 
    % the pseudo-semantic prior, sample reweighting, and input transformation, respectively.
    % PSP refers to training a UAP using semantic samples drawn from a pseudo-semantic prior.
    % \chany{RP and PSP refer to training a UAP using random noises and semantic samples drawn from random prior and pseudo-semantic prior, respectively.}
    }
    % $FR$ (\%) of various models on the UAP generated on ResNet152. }  
    \vspace{-0.2cm}
    \label{fig:ablation_1}
\end{figure}


\subsection{Ablation Study} We conduct ablation experiments to explore the effectiveness of the proposed pseudo-semantic prior, sample reweighting, and applying input transformation techniques on the semantic samples.
In the following experiments, we generate UAPs on ResNet152 and evaluate them across various CNN models (\eg, AlexNet, VGG16, VGG19, ResNet152, and GoogleNet).

% 1. SP, SP+reweight, SP+transform, SP+reweight+transform을 resnet152로 만들어서 alex~googlenet에 대해 $FR$ 그래프 만들기
% 2. googlenet과 resnet152를 사용해 random noise를 10장 만들고, input transform을 했을 때 성능 보여주기
% 3. crop and resize하는 개수 N을 1, 2, 5, 10으로 해서 성능 그래프 만들기. 이거는 vgg19 and resnet152?
\vspace{-0.2cm}
\paragraph{Impact of Each Proposed Component.} %In this experiment,
%to check the effect of each proposed component, we generate the UAP on ResNet152 and evaluate it on various CNN models. 
% in Figure.
We investigate how each component of PSP-UAP such as pseudo-semantic prior, sample reweighting, and input transformation affects attack performance.
For a fair comparison, we assign the number of random noises and semantic samples to 10.
As shown in Figure~\ref{fig:ablation_1}, our pseudo-semantic prior method achieves a higher $FR$ rather than random prior when used as an input prior.
%Additionally, applying sample reweighting on the semantic samples improves $FR$s in both white-box and black-box attacks.
%Incorporating input transformation into semantic samples further enhances black-box attack transferability.
%However, the white-box $FR$ on ResNet152 decreases in PSP-T compared to PSP, as transformations applied to the semantic samples do not guarantee content retention.
%Such inconsistency may reduce their effectiveness as meaningful data samples for training.
%This issue is addressed by integrating sample reweighting into the transformation technique in our final method, as shown in Figure~\ref{fig:ablation_1}.
%These findings indicate that the sample reweighting method not only mitigates this limitation but also achieves the highest white-box $FR$.
Additionally, applying sample reweighting to the semantic samples improves the $FR$ in both white-box and black-box attacks.
Incorporating input transformation into semantic samples enhances the attack performance.
Remarkably, combining both sample reweighting and input transformation yields the greatest overall performance improvement. 
%This approach plays a significant role in enhancing effectiveness in both white-box and black-box attack scenarios.
%By combining pseudo-semantic prior, sample reweighting, and input transformation, PSP-UAP achieves the highest $FR$ across all models.

\vspace{-0.2cm}
% \paragraph{Input Transformation to Other Data-free UAP.} 
 
% We evaluate the effect of applying input transformations to semantic samples in our method against random noise within TRM-UAP~\cite{TRM}, using the same transformation $T(\cdot)$.
% To ensure a fair evaluation, we set the number of samples $N=10$ for both random noise and semantic samples.
% Figure~\ref{fig:ablation_2} shows that the $FR$ of TRM-UAP decreases when input transformations are applied.
% In contrast, applying transformations to semantic samples drawn from our pseudo-semantic prior increases the $FR$ compared to using semantic samples alone.
% We believe this improvement results from the richer semantic content in our pseudo-semantic prior compared to random noise, enabling the UAP to learn a wider variety of patterns through input transformations.

\paragraph{Expanding Pseudo-semantic Prior as a Universal Strategy.}
We evaluate the scalability of the pseudo-semantic prior (PSP) as a universal strategy to validate its effectiveness.
To ensure a fair evaluation, we set the number of samples $N=10$ for both random noise and semantic samples.
In Figure~\ref{fig:ablation_2}, we first apply input transformation to random noise within TRM-UAP~\cite{TRM} and GD-UAP~\cite{gd-uap}, using the same transformation $T(\cdot)$, which results in performance degradation.
However, the integration of PSP with GD-UAP and TRM-UAP for input transformation leads to a significant improvement in attack performance.
Furthermore, each baseline achieves the highest $FR$ when combined with our full method, including sample reweighting.
We believe that this improvement results from the richer semantic content in our pseudo-semantic prior compared to random noise, enabling the UAP to learn a wider variety of patterns through input transformation.


\begin{figure}[t]
\centering
    \includegraphics[width=\linewidth]{figure_sup/ablation_c_only.pdf}
    \caption{Demonstrating that PSP serves as a universal strategy to other data-free UAP methods. Avgerage fooling rate (\%) refers average FR (\%) on AlexNet, VGG16, VGG19, ResNet152, and GoogleNet, with UAP crafted on ResNet152. P, T, and RW denot PSP, input transformation, and sample reweighting, respectively.}
    
    % Performance Comparison of UAPs generated by applying transformations to random noise with TRM-UAP~\cite{TRM} and to semantic samples from the pseudo-semantic priors in our method.
    % Comparison of UAP performance when applying transformations to random noise with TRM-UAP~\cite{TRM} and to semantic samples from pseudo-semantic priors in our method.
    % $T$ indicates the use of input transformations. All UAPs are generated on ResNet152.
      
    %proposed $FR$ (\%) of various models on the UAP generated on ResNet152. RP and PSP refer to using random prior and pseudo-semantic prior to generate training data samples, respectively. $T$ denotes the application of input transformations in each case.}   
    \label{fig:ablation_2}
    \vspace{-0.2cm}
\end{figure}

\paragraph{The Number of Semantic Samples.} 
We report the attack performance with respect to the number of samples $N$ in Figure~\ref{fig:ablation_num} to analyze the impact of the sample size on our method.
Empirically, we set $N=10$ as it achieves the highest attack performance, though results show generally stable performances across different sample sizes.
Notably, even with $N=1$, our method achieves superior attack performance compared to other data-free methods.

% \chany{
% \paragraph{Hyperparameter analysis.}
% We report the impact of hyperparameters for input transformation and the number of semantic samples.
% For input transformation, we perform a comparative analysis on ResNet152 with $\theta \in \{3,6,9,12\}$, $\beta_{high} \in \{2,4,6,8\}$, and $m \in \{2,3,4,5\}$ to determine the optimal parameter values, extending the evaluation across other models.
% Each transformation experiment is conducted independently to isolate and analyze its impact on attack performance.
% Based on the analysis in Figure~\ref{fig:ablation_num}, we set $\theta=6$, $\beta_{high}=4$, and $m=2$ in our experiments.
% Moreover, we set $N=10$ as it achieves the highest attack perfoemance, though results show generally stable performances across different sample sizes.
% Notably, even with $N=1$, our method achieves superior attack performance compared to other data-free methods.
% }

%PSP-UAP is trained with $N$ semantic samples to reduce the randomness since they are generated by sampler $\mathcal{C}$ in Eq.~\eqref{crop_resize}.
%As shown in Figure~\ref{fig:ablation_num}, PSP-UAP with already achieves higher transferability than other data-free methods.
%Existing data-free methods are only using random noise as training data.
%These results show that leveraging even a single semantic sample in training significantly enhances transferability.
%As we increase $N$, $FR$ also rises and stabilizes when $N>10$.
%Hence, we set $N=10$ in our experiments.

\paragraph{UAP Visualization.}
In Figure~\ref{fig:uaps}, we visualize the UAPs at each training iteration to verify that the pseudo-semantic prior, constructed from UAPs in the training phase, captures a variety of inherent patterns.
We observe that the UAPs contain more diverse patterns in the early stages of training.
We believe this variability allows us to obtain semantic samples with a broad range of patterns, through which the UAP learns diverse semantic representations.

\begin{figure}[t]
\centering
    \includegraphics[width=\linewidth]{figures/hyper.pdf}
    \caption{
    Ablation study on the hyperparameters for input transformation and $N$. The $FR$ (\%) of UAPs generated with different values of hyperparameters are evaluated across various models.}
    \label{fig:ablation_num}
    \vspace{-0.255cm}
\end{figure}

% \vspace{-1.0cm}
%\input{table/black_box_alex_final}

==> table/HIT.tex <==
% \begin{table}[t]
%   \centering
%   \footnotesize % 글꼴 크기 줄이기
%   \setlength{\tabcolsep}{0.8pt} % 열 간격 줄이기
%   \renewcommand{\arraystretch}{1.1} % 행 높이 조정
%   \begin{tabular}{lccc c}
%     \toprule
%     Attack & VGG19 & ~DenseNet121 & ~MobileNet-v2 & Avg.\\
%     \midrule
%     HIT & 53.57 &~ 58.38 & ~53.86 & ~39.94*  \\
%     PSP & \textbf{56.74} & ~\textbf{73.62} &~ \textbf{69.41} & ~\textbf{58.61}*  \\
%     \bottomrule
%   \end{tabular}
%   \caption{Robustness evaluation of our method and TRM against JPEG compression and ensemble adversarially trained models.}
%   %\vspace{-0.6cm}
%   \label{tab:HIT}
% \end{table}

% \begin{table}[t]
%   \centering
%   \scriptsize % 글꼴 크기 줄이기
%   \setlength{\tabcolsep}{2.5pt} % 열 간격 줄이기
%   \renewcommand{\arraystretch}{1.1} % 행 높이 조정
%   \begin{tabular}{cccccc}
%     \toprule
%     $\delta_\infty$ constraint & Attack & VGG19 & ~DenseNet121 & ~MobileNet-v2 & Avg. \\
%     \midrule
%     \multirow{2}{*}{$\epsilon=8$}
%     &HIT & 37.64 & 40.80 &  \textbf{69.90} &  46.13 \\
%     &PSP & \textbf{69.76} & \textbf{52.60} & 61.12&  \textbf{61.16}  \\
%     \hline
%     \multirow{2}{*}{$\epsilon=16$}
%     &HIT & 94.75 & 88.81 & \textbf{97.81} & 93.79 \\
%     &PSP & \textbf{97.79} & \textbf{94.58} & 95.51 & \textbf{95.96} \\
%     \bottomrule
%   \end{tabular}
%   \caption{Comparison between HIT and our method under diverse $\epsilon$ constraints.}
%   \vspace{-0.3cm}
%   \label{tab:convnext_vit}
% \end{table}



\begin{table}[h]
  \centering
  \scriptsize % 글꼴 크기 줄이기
  \setlength{\tabcolsep}{2.5pt} % 열 간격 줄이기
  \renewcommand{\arraystretch}{0.95} % 행 높이 조정
  \begin{tabular}{c|c|cccc}
    \hline
    Attack & $\epsilon$ & VGG19 & ~DenseNet121 & ~MobileNet-v2 & Avg. \\
    \hline
    HIT & \multirow{2}{*}{$\frac{8}{255}$ / $\frac{16}{255}$} & 37.64 / 94.75  & 40.80 / 88.81 &  \textbf{69.90} / \textbf{97.81}&  46.13 / 93.79\\
    Ours & & \textbf{69.76} / \textbf{97.79} & \textbf{52.60} / \textbf{94.58} & 61.12 / 95.51 &  \textbf{61.16} / \textbf{95.96} \\
    \hline
    % \multirow{2}{*}{$\epsilon=16$}
    % &HIT & 94.75 & 88.81 & \textbf{97.81} & 93.79 \\
    % &PSP & \textbf{97.79} & \textbf{94.58} & 95.51 & \textbf{95.96} \\
    % \hline
  \end{tabular}
  \vspace{-0.2cm}
  \caption{\scriptsize{Comparison with HIT [A3] under different $\epsilon$ constraints in Eq.(2). We select only target models that overlap with our experiments.}}
  \vspace{-0.5cm}
  \label{tab:hit}
\end{table}

==> table/ablation.tex <==
\begin{table}[hb]
  \centering
  \footnotesize
  %\scriptsize % 글꼴 크기 줄이기
  \setlength{\tabcolsep}{1.1pt} % 열 간격 줄이기
  \renewcommand{\arraystretch}{1} % 행 높이 조정
\begin{tabular}{lcccccc}
    \toprule
    Model & Transform & AlexNet & VGG16 & VGG19 & RN152 & GoogleNet \\ 
    \midrule
    \multirow{4}{*}{RN152}  & $p_{\boldsymbol{z}}$(w/o $T$)& 32.28 & 54.58 & 51.71 & 47.57 & 33.32 \\
                                & $p_{\boldsymbol{z}}$(with $T$) & 40.12 & 58.60 & 56.07 & 43.26 & 38.33\\ 
                                & $p_{\mathbf{x}}$(w/o $T$) & 48.24 & 79.17 & 79.41 & 78.17 & 61.93 \\
                                & $p_{\mathbf{x}}$(with $T$) & 53.63 & 82.31 & 82.73 & 67.02 & 65.84 \\ 
    \cmidrule(lr){1-7} % horizontal line separating sections

    \multirow{4}{*}{GoogleNet} & $p_{\boldsymbol{z}}$(w/o $T$) & 57.40 & 74.59 & 75.25 & 53.33 & 79.02 \\
                               &$p_{\boldsymbol{z}}$(with $T$) & 58.12 & 75.11 & 75.46 & 53.16 & 79.06 \\ 
                               & $p_{\mathbf{x}}$(w/o $T$) & 57.62 & 76.92 & 74.47 & 54.56 & 82.23 \\
                               & $p_{\mathbf{x}}$(with $T$)& 61.45 & 78.28 & 79.31 & 58.48 & 83.00 \\ 
    \bottomrule
\end{tabular}
  \caption{Transferability results of applying input transformation to random noise and semantic samples. $p_{\boldsymbol{z}}$ and $p_{\boldsymbol{z}}$ refer to using random noise and semantic samples as training data, respectively, while $T$ denotes the application of input transformations in each case.}
  \label{tab:ablation_2}
\end{table}


==> table/black_box_alex_final.tex <==
\begin{table*}[t]
\footnotesize
  \centering
  \begin{tabular}{cccccccc}
    \toprule
    Model & Attack & AlexNet~~ & VGG16~~ & VGG19~~ & ResNet152~~ & GoogleNet~~ & Average\\
    \midrule
    \multirow{4}{*}{AlexNet} 
    & AT-UAP-U & \textbf{96.66}\scriptsize{$\pm$0.12}* & {72.33}\scriptsize{$\pm$0.50}~~ & {67.24}\scriptsize{$\pm$0.18}~~ & {43.63}\scriptsize{$\pm$0.29}~~ & {62.01}\scriptsize{$\pm$0.32}~~ & {68.37}\\
    & TRM-UAP & 93.53\scriptsize{$\pm$0.07}* & 60.10\scriptsize{$\pm$0.24}~~ & 57.08\scriptsize{$\pm$0.15}~~ & 27.31\scriptsize{$\pm$0.30}~~ & 32.70\scriptsize{$\pm$0.22}~~ & 54.14 \\
    & \textbf{PSP-UAP (Ours)} & 93.20\scriptsize{$\pm$0.23}* & \textbf{79.52}\scriptsize{$\pm$0.47}~~ & \textbf{75.81}\scriptsize{$\pm$0.47}~~ & \textbf{50.40}\scriptsize{$\pm$1.01}~~ & \textbf{67.02}\scriptsize{$\pm$0.73}~~ & \textbf{73.19 }\\

    & \textbf{PSP-UAP (resize 1)} & 91.77\scriptsize{$\pm$0.32}* & \textbf{76.56}\scriptsize{$\pm$0.67}~~ & \textbf{74.07}\scriptsize{$\pm$0.54}~~ & \textbf{49.20}\scriptsize{$\pm$1.12}~~ & \textbf{66.00}\scriptsize{$\pm$0.75}~~ & \textbf{71.52 }\\
    \hline
    
    \multirow{4}{*}{VGG16} 
    & AT-UAP-U & \textbf{54.15}\scriptsize{$\pm$0.70}~~ & 94.50\scriptsize{$\pm$0.21}* & 86.65\scriptsize{$\pm$0.70}~~ & 36.96\scriptsize{$\pm$1.03}~~ & 48.53\scriptsize{$\pm$1.32}~~ & 64.16 \\
    & TRM-UAP & 47.53\scriptsize{$\pm$0.51}~~ & 94.30\scriptsize{$\pm$0.12}* & 89.68\scriptsize{$\pm$0.14}~~ & {61.43}\scriptsize{$\pm$0.40}~~ & 53.95\scriptsize{$\pm$0.59}~~ & {69.38}\\
    & \textbf{PSP-UAP (Ours)} & {49.19}\scriptsize{$\pm$0.42}~~ & \textbf{96.01}\scriptsize{$\pm$0.07}* & \textbf{92.62}\scriptsize{$\pm$0.13}~~ & \textbf{70.48}\scriptsize{$\pm$0.97}~~ & \textbf{59.29}\scriptsize{$\pm$0.80}~~ & \textbf{73.52 }\\

    & \textbf{PSP-UAP (resize 1)} & {49.19}\scriptsize{$\pm$0.42}~~ & \textbf{96.01}\scriptsize{$\pm$0.07}* & \textbf{92.62}\scriptsize{$\pm$0.13}~~ & \textbf{70.48}\scriptsize{$\pm$0.97}~~ & \textbf{59.29}\scriptsize{$\pm$0.80}~~ & \textbf{73.52 }\\
    
    \hline
    
    \multirow{4}{*}{VGG19} 
    & AT-UAP-U & \textbf{62.05}\scriptsize{$\pm$1.01}~~ & 88.96\scriptsize{$\pm$0.50}~~ & 92.85\scriptsize{$\pm$0.48*} & 42.72\scriptsize{$\pm$0.51}~~ & \textbf{60.99}\scriptsize{$\pm$1.41}~~ & 69.51\\
    & TRM-UAP & 46.01\scriptsize{$\pm$0.44}~~ & 89.82\scriptsize{$\pm$0.15}~~ & 91.35\scriptsize{$\pm$0.30}* & 47.19\scriptsize{$\pm$0.46}~~ & 46.48\scriptsize{$\pm$0.78}~~ & 64.17\\
    & \textbf{PSP-UAP (Ours)} & 48.93\scriptsize{$\pm$0.72}~~ & \textbf{94.55}\scriptsize{$\pm$0.14}~~ & \textbf{94.65}\scriptsize{$\pm$0.10}* & \textbf{67.13}\scriptsize{$\pm$1.37}~~ & {58.83\scriptsize{$\pm$1.19}}~~ & \textbf{72.81}\\

    & \textbf{PSP-UAP (resize 1)} & 48.93\scriptsize{$\pm$0.72}~~ & \textbf{94.55}\scriptsize{$\pm$0.14}~~ & \textbf{94.65}\scriptsize{$\pm$0.10}* & \textbf{67.13}\scriptsize{$\pm$1.37}~~ & {58.83\scriptsize{$\pm$1.19}}~~ & \textbf{72.81}\\

    \hline
    
    \multirow{4}{*}{ResNet152} 
    & AT-UAP-U & 49.78\scriptsize{$\pm$0.68}~~ & 62.78\scriptsize{$\pm$0.71}~~ & 60.54\scriptsize{$\pm$0.49}~~ & 73.15\scriptsize{$\pm$1.15}* & 48.37\scriptsize{$\pm$0.49}~~ & 58.92\\
    & TRM-UAP & {53.56}\scriptsize{$\pm$0.75}~~ & 77.20\scriptsize{$\pm$0.35}~~ & 73.30\scriptsize{$\pm$0.41}~~ & 67.46\scriptsize{$\pm$0.35}* & 57.54\scriptsize{$\pm$0.50}~~ & 65.81\\
    & \textbf{PSP-UAP (Ours)} & \textbf{55.29}\scriptsize{$\pm$0.87}~~ & \textbf{85.62}\scriptsize{$\pm$1.60}~~ & \textbf{85.79}\scriptsize{$\pm$0.92}~~ & \textbf{83.61}\scriptsize{$\pm$2.06}* & \textbf{71.14}\scriptsize{$\pm$1.27}~~ & \textbf{76.29}\\

    & \textbf{PSP-UAP (resize 1)} & 58.82\scriptsize{$\pm$1.17}* & \textbf{88.59}\scriptsize{$\pm$1.38}~~ & \textbf{87.35}\scriptsize{$\pm$0.92}~~ & \textbf{85.65}\scriptsize{$\pm$1.70}~~ & \textbf{76.00}\scriptsize{$\pm$1.33}~~ & \textbf{79.28 }\\
    \hline
    
    \multirow{4}{*}{GoogleNet} 
    & AT-UAP-U & 55.65\scriptsize{$\pm$0.37}~~ & 71.38\scriptsize{$\pm$0.83}~~ & 68.25\scriptsize{$\pm$0.59}~~ & 43.03\scriptsize{$\pm$0.42}~~ & 82.60\scriptsize{$\pm$0.72}* & 64.58\\
    & TRM-UAP & 60.10\scriptsize{$\pm$1.16}~~ & \textbf{79.66}\scriptsize{$\pm$0.95}~~ & \textbf{79.98}\scriptsize{$\pm$1.06}~~ & 58.85\scriptsize{$\pm$1.94}~~ & \textbf{85.32}\scriptsize{$\pm$0.04}* & 72.78\\
    & \textbf{PSP-UAP (Ours)} & \textbf{62.78}\scriptsize{$\pm$0.41}~~ & 79.37\scriptsize{$\pm$0.35}~~ & 79.87\scriptsize{$\pm$0.15}~~ & \textbf{59.12}\scriptsize{$\pm$0.14}~~ & 84.16\scriptsize{$\pm$0.26}* & \textbf{73.06}\\

    & \textbf{PSP-UAP (resize 1)} & 65.22\scriptsize{$\pm$0.56}* & \textbf{78.43}\scriptsize{$\pm$0.73}~~ & \textbf{79.26}\scriptsize{$\pm$0.73}~~ & \textbf{57.63}\scriptsize{$\pm$0.66}~~ & \textbf{81.43}\scriptsize{$\pm$0.49}~~ & \textbf{72.39 }\\
    \bottomrule
  \end{tabular}
  \caption{Black-box attack transferability of the UAP synthesized by our PSP-UAP method compared to other data-free universal attacks. We show the mean and standard deviation of $FR$ with five runs. Bold $FR$ (\%) denotes the best performance. The UAPs are crafted on AlexNet, VGG16, VGG19, ResNet152, and GoogleNet. * indicate $FR$ of the white-box model. }
  \label{tab:black_box_combined_final}
\end{table*}

